NetQASM -- A low-level instruction set architecture for hybrid quantum-classical programs in a quantum internet

We introduce NetQASM, a low-level instruction set architecture for quantum internet applications. NetQASM is a universal, platform-independent and extendable instruction set with support for local quantum gates, powerful classical logic and quantum networking operations for remote entanglement generation. Furthermore, NetQASM allows for close integration of classical logic and communication at the application layer with quantum operations at the physical layer. This enables quantum network applications to be programmed in high-level platform-independent software, which is not possible using any other QASM variants. We implement NetQASM in a series of tools to write, parse, encode and run NetQASM code, which are available online. Our tools include a higher-level SDK in Python, which allows an easy way of programming applications for a quantum internet. Our SDK can be used at home by making use of our existing quantum simulators, NetSquid and SimulaQron, and will also provide a public interface to hardware released on a future iteration of Quantum Network Explorer.

==> Makefile <==
TEX_FLAGS = ""
TEX       = pdflatex ${TEX_FLAGS}
NAME      = netqasm
MAIN      = ${NAME}.tex
PDF       = ${NAME}.pdf

pdf:
	${TEX} ${MAIN}

pdf-twice:
	${TEX} ${MAIN}
	${TEX} ${MAIN}

bibtex:
	bibtex ${NAME}

clean:
	find . \( -name '*.aux' -o -name '*.bbl' -o -name '*.out' -o -name '*.end' \) -delete

open:
ifeq (, $(shell which open 2> /dev/null))
	xdg-open ${PDF}
else
	open ${PDF}
endif


all: pdf bibtex pdf-twice

